Triple Patterning Lithography (TPL) Layout Decomposition using End-Cutting

Triple patterning lithography (TPL) is one of the most promising techniques in the 14nm logic node and beyond. However, traditional LELELE type TPL technology suffers from native conflict and overlapping problems. Recently LELEEC process was proposed to overcome the limitations, where the third mask is used to generate the end-cuts. In this paper we propose the first study for LELEEC layout decomposition. Conflict graphs and end-cut graphs are constructed to extract all the geometrical relationships of input layout and end-cut candidates. Based on these graphs, integer linear programming (ILP) is formulated to minimize the conflict number and the stitch number.

==> doc/abstract_long.tex <==

\section{Abstract}

As the semiconductor process further scales down, the industry encounters many lithography-related issues.
In the 14nm logic node and beyond, triple patterning lithography (TPL) is one of the most promising techniques,
because of the delay of other candidates, such as extreme ultraviolet lithography (EUVL) and electron beam lithography (EBL) \cite{TPL_SPIE2012_Lucas}.

\begin{figure}[tb]
  \centering
  \hspace{.1in}
  \subfigure[]{\includegraphics[width=0.18\textwidth]{0Label_TPL}}
  \hspace{.1in}
  \subfigure[]{\includegraphics[width=0.24\textwidth]{1Target}}
  \hspace{.1in}
  \subfigure[]{\includegraphics[width=0.24\textwidth]{2LELELE}}
  \caption{Process of LELELE~(a) Some labels.~(b) Target features.~(c) Decomposed layout with one conflict introduced.}
  \label{fig:LELELE}
  \vspace{-.1in}
\end{figure}

One traditional process of TPL is with the same principle of litho-etch-litho-etch (LELE) type double patterning lithography (DPL),
where the original layout is decomposed into three masks and manufactured through three exposure/etching steps.
This technology is called LELE-litho-etch (LELELE).
Many research has been carried out to solve the corresponding design problems, including layout decomposition
\cite{TPL_SPIE08_Cork,TPL_ICCAD2011_Yu,TPL_SPIE2011_Ghaida,TPL_DAC2012_Fang} and routing \cite{TPL_DAC2012_Ma,TPL_2012_Lin}.
However, even with stitch insertion, there are some native conflicts in LELELE.
Fig. \ref{fig:LELELE} shows a 4-clique conflicts among features $a$, $b$, $c$, and $d$.
Since this 4-clique structure is common in advanced standard cell design, LELELE type TPL still suffers from the native conflict problem \cite{TPL_ICCAD2011_Yu}.
Besides, compared with LELE, there are more serious overlapping problem in LELELE \cite{TPL_SPIE08_Ausschnitt}.

To overcome all these limitations derived from LELELE, recently Lin \cite{TPL_ISPD2012_Lin} proposes a new TPL manufacturing process, called LELE-end-cutting (LELEEC).
As a TPL, this new manufacturing process contains three mask steps, namely first mask, second mask, and \textit{trim} mask.
Fig. \ref{fig:LELEEC} illustrates an example of the LELEEC process.
To generate the target features in Fig. \ref{fig:LELEEC}(b), the first and second masks are used for pitch splitting,
which is similar to LELE process in DPL.
These two masks are shown in Fig. \ref{fig:LELEEC}(c).
Finally, trim mask is used to trim out the desired region as shown in Fig. \ref{fig:LELEEC}(d).
The trim mask is used to generate some end-cuts to further split feature patterns.
It shall be noted that since these end-cuts are printed through one mask, some end-cuts may not be compatible to each other.
As a result, the features that is not LELELE-friendly can be printed without introducing any conflict through the LELEEC process.

Layout decomposition, which is the most crucial step for TPL, has been extremely studied under LELELE process 
\cite{TPL_SPIE08_Cork,TPL_ICCAD2011_Yu,TPL_SPIE2011_Ghaida,TPL_DAC2012_Fang}.
However, because of the trim mask and the end-cutting process, the layout decomposition for LELEEC is still an open problem.
The difficults of the new layout decomposition problem lie on the following two-fold:
(1) Since some end-cuts are not compatible, the design of trim mask is crucial.
(2) How to model the overlapping errors, especially the errors caused by trim mask in this process is also unknow.

\begin{figure}[tb]
  \centering
  \subfigure[]{\includegraphics[width=0.18\textwidth]{0Label_TPLEC}}
  \hspace{.1in}
  \subfigure[]{\includegraphics[width=0.24\textwidth]{1Target}}
  \hspace{.1in}
  \subfigure[]{\includegraphics[width=0.24\textwidth]{2LELE}}
  \hspace{.1in}
  \subfigure[]{\includegraphics[width=0.24\textwidth]{3Trim}}
  \caption{Process of LELEEC~(a) Some labels.~(b) Target features.~(c) First and second mask patterns.~(d) Trim mask, and final decomposition without conflict.}
  \label{fig:LELEEC}
  \vspace{-.1in}
\end{figure}

In this paper, we propose the first study for LELEEC layout decomposition.
Given a layout which is specified by features in polygonal shapes, we extract the geometrical relationships and construct the conflict graphs.
Furthermore, the compatibility of all end-cuts candidates are also modeled in the conflict graphs.
Based on the conflict graphs, integer linear programming (ILP) is formulated to assign each vertex into one layer.
Our goal in the layout decomposition is to minimize the conflict number, and at the same time minimize the overalpping errors.


